A Starter's Kit for Concentric Tube Robots

Concentric Tube Robots (CTRs) have garnered significant interest within the surgical robotics community because of their flexibility, dexterity, and ease of miniaturization. However, mastering the unique kinematics and design principles of CTRs can be challenging for newcomers to the field. In this paper, we present an educational kit aimed at lowering the barriers to entry into concentric tube robot research. Our goal is to provide accessible learning resources for CTRs, bridging the knowledge gap between traditional robotic arms and these specialized devices. The proposed kit includes (1) An open-source design and assembly instructions for an economical (cost of materials $\approx$ 700 USD) modular CTR; (2) A set of self-study materials to learn the basics of CTR modeling and control, including automatically-graded assignments. To evaluate the effectiveness of our educational kit, we conducted a human subjects study involving first-year graduate students in engineering. Over a four-week period, participants -- none of whom had any prior knowledge of concentric tube robots -- successfully built their first CTR using the provided materials, implemented the robot's kinematics in MATLAB, and conducted a tip-tracking experiment with an optical tracking device. Our findings suggest that the proposed kit facilitates learning and hands-on experience with CTRs, and furthermore, it has the potential to help early-stage graduate students get rapidly started with CTR research. By disseminating these resources, we hope to broaden participation in concentric tube robot research to a wider a more diverse group of researchers.

==> related_work.tex <==
\section{RELATED WORK}
\label{sec:related}
% In recent years, there have been advances in CTR research that aim to make the field more accessible to newcomers. Here we will discuss advances in tube manufacturing techniques and developments in actuation modules. 


%In this section we discuss the and highlight the key features of the state-of-the-art prototypes  in the research community that drive the need for an open-source platform for teaching and building CTRs. 
%It is shown in ~\cite{Nwafor2023,Grassmann2020} that the most research groups working on CTR technologies are focused on developing prototypes over a robotic platform. 

% \textit{A. Tube Materials and Manufacturing}
\subsection{Tube Materials and Manufacturing}

% Traditionally, the tube structures in CTRs were constructed exclusively from Nitinol -- a super-elastic material that flexes predictably and resists permanent deformation ~\cite{Gilbert2016, dupont2009design, torabi2014compact}. This property is important for CTRs because it enables the pre-curved tubes to repeatedly interact with each other without any permanent changes in shape. Despite the utility of Nitinol, the cost of stock material is high, and the procedures to produce pre-curved tubes from stock tubing require specialized furnaces that can reach temperatures in the range of $440-550^{\circ}$C) ~\cite{Nwafor2023, torabi2014compact, kim2014toward, shrivastava_medical_2004}. 

%Nwafor \textit{et al}.~\cite{Nwafor2023} report 24 different publications that use furnace shape-setting for Nitinol, many with their own customized variation of the procedure. 

Motivated by these challenges, researchers have begun investigating alternative materials and manufacturing methods for pre-curved tubes. Most of the alternative materials are plastic since they are generally lower in cost than Nitinol. To create shaped tubes, researchers have developed procedures using additive manufacturing ~\cite{morimoto2016design, amanov2015additive} and heat-setting. While the heat setting procedure is similar to the process for Nitinol, setting plastic materials requires much lower temperatures and simpler equipment. Recently, Lu \textit{et al.} in~\cite{Lu2023} proposed a method that uses Nylon-12 medical tubing and custom molds to heat-set the tubes to desired pre-curvatures. We discuss this procedure in further detail in Section \ref{sec:design}.

%Most CTR’s use nitinol as the choice of material for the tubes used in their devices~\cite{Gilbert2016, dupont2009design, torabi2014compact}  due to its super-elastic properties. Despite the versatility of nitinol for this application, this may also act a barrier to developing a standardised platform, because existing techniques require large furnaces, and they are very easily accessible~\cite{torabi2014compact, kim2014toward}. Therefore, there are on-going attempts where groups have tried various fabrication techniques involving the use of thermoplastic polymers to fabricate tubes for CTRs~\cite{morimoto2016design, amanov2015additive}. Additive manufacturing opens a lot of avenues in this respect, giving the researchers a plethora options for material selection and fabrication methodologies. Lu et al. in~\cite{Lu2023} propose a method that uses Nylon 12 medical tubing and custom molds  to heat-set the tubes to desired pre-curvatures. We discuss in further detail in Section III.

% \textit{B.	Actuation modules}
\subsection{Actuation modules}
Actuation modules drive the translation and rotation of each tube with respect to the others (Fig. \ref{fig:robot-system}). Nwafor \textit{et al.} conducted a review of all existing CTR actuation modules and found 64 different designs. Grassman \textit{et al.} establish that this tendency to design actuation modules for specific uses is forcing researchers to reinvent the wheel for each experiment. Some existing CTR actuation modules were designed to be adapted to a different number of tubes or tools (e.x. \cite{morimoto2016design, wang2020design}, but only Grassman \textit{et a.}~\cite{grassmann2024open} have designed and released a truly open-source CTR actuation module design. 

Grassman \textit{et al}. proposed an open-source, modular actuation system for a variety of continuum robots, including concentric tube robots. Like other modular CTR actuation devices, translation and rotation of each tube is completely decoupled, and each tube requires one actuation stage that controls both translation and rotation. This system uses brushless DC motors and a low-gear ratio transmission that enables proprioceptive torque sensing by measuring motor currents. Because this device is capable of torque sensing, users can implement high-speed torque control. 
%%
Along with reporting the experiments they conducted with this device, the researchers released assembly guides and BOMs so that other researchers could also build this device. However, the price of materials for a two-tube CTR actuation system is \$1,785 (2023 USD), not including materials or equipment for tube manufacturing. This device is an important step towards creating open-source devices for aspiring CTR researchers, but the price point is still relatively high for a starting device or a classroom tool. 

%Actuation modules allow  the CTRs to translate and rotate the tubes with respect to one another. Conventionally, CTRs have one module for every tube in the robot and these modules have two members which control the translation and rotation of that tube. In each module the translation and rotational members are linked to the proximal end of the tube either directly or indirectly. Most actuation modules have the have the rotational and translational members decoupled. CTRs can also have their actuation modules mechanically linked, but most implementations don’t have them linked, and reserve the option to have them linked using software limits ~\cite{Nwafor2023}.  As each module has two degrees of freedom (translation and rotation), they consist of two or more actuators. These actuators are usually DC motors and tend to be coupled with an encoder for implementing position control~\cite{Gilbert2016, dupont2009design, torabi2014compact}. Torque control algorithms avoid extra sensors by use motor current for feedback, but the difference in cost is dependent on the encoder and application~\cite{ellin2008design}.

%Grassmann et al. propose a modular device to address the lack of a standardized platform in~\cite{grassmann2024open}, which aims to create an open-source tool for creating continuum robots of different modalities. Their research focuses mainly on the hardware design of the new platform which revolves around the modular design of their actuation unit. This actuation unit uses a Brushless DC  (BLDC) motor and encoder pair for controlling a degree of freedom. This increases the cost of the actuation module as BLDCs have a high entry-price point~\cite{derammelaere2016quantitative}. 

In this paper, we present a full concentric tube robot, including an actuation module based on ~\cite{wang2020design, grassmann2024open, bruns2021modular} and example tubes based on ~\cite{Lu2023}. This system consists of easy to source components and several custom components that are designed to be 3D printed or laser cut. Our main contributions include:

\begin{enumerate}
    \item An open-source design for an inexpensive, modular concentric tube robot that is appropriate for both research and education
    \item A full system validation that proves our device is usable for precise kinematic verification experiments 
    \item A user study that demonstrates the usability of our open-source materials for graduate students 
\end{enumerate}

%Adapting the method in~\cite{Lu2023} for fabricating tubes and using the designs in~\cite{grassmann2024open, wang2020design, bruns2021modular} as an inspiration, we have put-forth a more complete robot design that focuses mainly on concentric tube robots. We also have made efforts to reduce the overall BOM cost of the robot as well as using easily available manufacturing techniques (e.g.: FDM 3D printing and Laser cutting) to make it more accessible to new researchers. Lastly,  a user study is conducted to validate the feasibility of our platform as an educational tool for the verification of kinematic models for CTRs  which is discussed in Section IV.


==> results.tex <==
\section{RESULTS}

% \subsection{Results of kinematic verification}
% This section reports the results of the error in the prediction of the forward kinematics model. The error is measured as an Root-Mean-Square Error (RMSE) between the robot tip positions. There are two models for the forward kinematics presented in \cite{webster_mechanics_2009}; a piece-wise constant curvature (PCC) model that assumes that the tubes are torsionally rigid and a model without this assumption, where an analytical solution (AS) for only a 2-tubed CTR is obtained using an energy minimisation approach.

% % The RMSE for a 2-tube CTR where the PCC and AS were used to model the forward kinematics was 7.0mm and 5.2mm respectively. When the same experiment was repeated after a few trials using the same set of tubes, the RMSE was 8.1 mm and 6.4 mm. Another experiment using three tubes was performed using the PCC model for the forward kinematics and the RMSE was 4.0 mm. Similarly, after a few trials, when the same experiment was run the RMSE was 5.6 mm.

% The results have been tabulated in table \ref{tabl:results}. The parameters of the two experiments are tabulated in table \ref{tab:joint_limits}.

% \begin{table}[t]
% \centering
% \caption{RMSE values for the two-tubed and three-tubed experiments.}
% % \setlength{\tabcolsep}{5pt} % Adjust the inter-column padding
% % \small
% \label{tabl:results}
% \begin{tabular}{@{}lccc@{}}
% \hline
%                       & \text{Two-tubes (PCC)} & \text{Two-tubes (AS)} & \text{Three-tubes (PCC)} \\ \hline
% \text{Fresh}        & 7.0mm              & 5.2mm             & 4.0mm              \\
% \text{Used}         & 8.1mm              & 6.4mm             & 5.6mm              \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Joint variable limits for the two-tubed and three-tubed experiments.}
% \label{tab:joint_limits}
% \small % or \footnotesize to make the font even smaller
% \setlength{\tabcolsep}{3pt} % Adjusts the space between columns
% \begin{tabular}{@{}lcc@{}}
% \hline
% Joint variable & \text{Two-tubes} & \text{Three-tubes} \\ \hline
% $\rho_1$       & $0 \leq \rho_1 \leq 40$ & $0 \leq \rho_1 \leq 40$ \\
% $\rho_2$       & $\rho_1 \leq \rho_2 \leq \rho_1 + 40$ & $\rho_1 \leq \rho_2 \leq \rho_1 + 40$ \\
% $\rho_3$       & NA & $\rho_2 \leq \rho_3 \leq \rho_2 + 40$ \\
% $\alpha_1$     & $-90 \leq \alpha_1 \leq 90$ & 0 \\
% $\alpha_2$     & $-90 \leq \alpha_2 \leq 90$ & 0 \\
% $\alpha_3$     & NA & 0 \\ \hline
% \end{tabular}
% \end{table}


\subsection{Results of user study}


\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.85\textwidth, trim=-1cm 0 -1cm -1cm,clip]{img/User_Study1.pdf}
    \caption{User reported CTR abilities before and after the study.}
    \label{fig: User-abilities}
\end{figure*}

Before beginning the survey, participants completed a pre-study survey so we could assess their prior knowledge and skills. We also collected basic demographic information.

We presented participants the following statement: ``Before beginning this study, I had prior academic, research, or industry experience with ()." We then provided them with the following options and asked them to select all options that applied for them: 3D printing, laser cutting, standard industrial robot kinematics, MATLAB, continuum robots, and concentric tube robots. All six participants had previous experience with standard industrial kinematics, and several had experience with 3D printing and MATLAB. No participants reported previous experience with continuum or concentric tube robots.

Due to time conflict during the study, one of the participants could not further contribute in the later technical modules. All the data reported in this work has been adjusted accordingly by removing the entry from this user.

At the beginning and end of the survey, we asked participants to rate their knowledge on a number of concentric tube robot topics that we covered over the course of the study. We presented the participants with the statement ``I know how to ()" to measure their ability.  From the beginning of the study to the end of the study and represented by Fig. \ref{fig: User-abilities}, we saw a significant increase in the participants’ confidence in their knowledge about CTR topics and abilities related to CTRs.

At the end of the user study, we also asked participants to rate the usability of the assembly guide and the kinematics assignments. For the assembly guides, we asked participants to rate the ease of use for each set of instructions and the ease of use for the entire system once assembled. For the kinematic assignments, we asked participants how useful different components of the assignments were for their learning. All participants either agreed or strongly agreed that the assembly guides provided sufficient instruction to construct the device and that the kinematics assignments advanced their understanding of CTR kinematics.






==> study_materials.tex <==
\section{Self-Study Materials}
We designed a set of learning materials that provide an introduction
to the kinematics of CTRs.
%%
These materials include readings, online assessments, and practical 
assignments.
%%

%%
The kinematics modeling approach covered in our materials is based on
the work of Webster~\cite{Webster2010}, and it is illustrated in 
Fig.~\ref{}.
%%



%%
% \section{KINEMATIC VERIFICATION}
% \label{sec: verification}
% We characterized the accuracy of our robot using a Polaris Vega  optical tracker (Northern Digital, Waterloo, ON, Canada). The setup for our experiment is shown in Fig. \ref{fig:fig-transform}. We tested both a two-tube setup and a three-tube setup. We defined the accessible joint positions for each experiment as shown in Table \ref{tab:joint_limits}. Note that the test with two tubes includes non-zero rotation limits while the three-tube experiment was conducted strictly in-plane. We moved the robot to 15 random positions sampled from the defined joint space and measured the actual position of the robot using the motion capture system. 

% We compared the ground truth data collected from the motion capture system to the expected end effector position as defined by the kinematics model presented by Webster \textit{et al.} in \cite{webster_mechanics_2009}. For tube curvatures, we used the \textit{measured curvature} values shown in Table \ref{tab: tube-parameters}. 

% %The root-mean-square error for the two-tube setup and three-tube setup were in range of 3-10.2mm and 3.5-7.5mm respectively. This error is comparable to the error reported for nylon tubes\cite{amanov2015additive} as well as Nitinol tubes \cite{Rucker2010}. 




% \begin{table}[b]
% \centering
% \caption{Joint variable limits for the two-tubed and three-tubed experiments.}
% \label{tab:joint_limits}
% \small % or \footnotesize to make the font even smaller
% \setlength{\tabcolsep}{3pt} % Adjusts the space between columns
% \begin{tabular}{@{}ccc@{}}
% \hline
% Joint variable & \text{Two-tubes} & \text{Three-tubes} \\ \hline
% $\rho_1$       & $0 \leq \rho_1 \leq 40$ & $0 \leq \rho_1 \leq 40$ \\
% $\rho_2$       & $\rho_1 \leq \rho_2 \leq \rho_1 + 40$ & $\rho_1 \leq \rho_2 \leq \rho_1 + 40$ \\
% $\rho_3$       & NA & $\rho_2 \leq \rho_3 \leq \rho_2 + 40$ \\
% $\alpha_1$     & $-90^\circ \leq \alpha_1 \leq 90^\circ$ & $0^\circ$ \\
% $\alpha_2$     & $-90^\circ \leq \alpha_2 \leq 90^\circ$ & $0^\circ$ \\
% $\alpha_3$     & NA & $0^\circ$ \\ \hline
% \end{tabular}
% \end{table}

% We defined error as the norm of the difference between the expected end effector position and the actual end effector position. For the two-tubes with rotation experiment, the RMSE ranged from 3.1 mm to 10.2 mm, with an average of 7.8 mm. For the three-tubes in-plane bending experiment, the RMSE ranged from 3.5 mm - 7.5 mm, with an average of 6.1 mm. Rucker \textit{et al.} \cite{Rucker2010} report an average of 2.91 mm of error in an experiment with two Nitinol tubes that underwent translation and rotation. To produce this result, they used parameter fitting on their collected data and kinematic model. We have not implemented any parameter fitting algorithms. Even so, our results with Nylon-12 tubes are comparable to results with Nitinol tubes. Similarly our results are also comparable to error reported for Nylon-12 tubes in \cite{amanov2015additive}.




% % The kinematics of concentric tube robots are often categorised into three workspaces: the joint space, the configuration space, and the task space. Therefore, there is a robot-dependent mapping from the joint space to configuration space and a robot-independent mapping from the configuration space to the task space. We implement the forward kinematics for concentric tube robots proposed in~\cite{webster_mechanics_2009} and verify the same using the NDI Polaris motion capture system. \WW{Since we are constantly referring to CTR Fkin in the later section, should we write out equation 13 and 14 on Webster's paper? I'm writing out those equations here just in case we need them somewhere.}


% % -------------- CTR twists and Fkin ----------------
% % \begin{align}
% % \begin{split}
% %     \xi_\phi &= [v^T_\phi \quad \omega^T_\phi] = [0 \quad 0 \quad 0 \quad 0 \quad 0 \quad 1]^T \\
% %     \xi_j(\mathbf{q}) &= [v_j^T \quad \omega_j^T] = [0 \quad 0 \quad 1 \quad \kappa_j(\mathbf{q}) \quad 0 \quad 0]^T
% %     \label{eqn:twists}
% % \end{split}
% % \end{align}

% % \begin{equation}
% %     g(\mathbf{q}) = \prod \limits_{j=1}^m e^{\left(\widehat{\xi_\phi}\left(\Delta\phi_j(q)\right)\right)} e^{\left(\widehat{\xi_j(q)}l_j(q)\right)}
% % \end{equation}
% % -------------- CTR twists and Fkin ----------------

% % % \textit{A.	Experiment setup and workflow}
% % \subsection{Experiment setup and workflow}

% % The kinematic model predicts the robot-tip position, as a function of the joint variables. The motion capture system tracks a needle pointer pointed at the robot-tip and a home frame attached to the robot. The coordinate system of the home frame is assigned such it is aligned with origin of the coordinate system that the kinematic model uses. Similarly, the coordinate frame of the needle pointer is assigned such that the origins of the needle pointer and the robot-tip coordinate frame are coincident. Fig.~\ref{fig:fig-transform} shows the frames of interest within the workspace.

% % % \textit{B.	Configuring the robot}
% % \subsection{Configuring the robot}

% % The kinematic model uses the start of the precurved section of the outermost tube of the CTR as the origin for the robot coordinate system. Therefore, we position the tubes such that the precurved sections of all the tubes are coincident to each other as well as the front plate of the robot. Using this as the reference, the tubes are aligned along the X-Z plane such that there is no twist with respect to each other. 
% % % Images in Fig… show how the tubes and robot should look like after being configured and set to home.

% % % \AR{Fig to have two images a and b, which are the front of the robot and the side view after homing}

% % % \textit{C.	Setting up the motion capture system}
% % \subsection{Setting up the motion capture system}

% % The motion capture system is the NDI Polaris Vega ST~\cite{NDI_Polaris_VegaST} which is a stereo camera setup. The camera has a working volume within which the tracking objects must be placed. For our experiments, we place the robot 45 inches or 120cm away from the camera to ensure that the robot and needle are within the field of view of the system. We use the API provided with the system to confirm that the tracking objects are visible to the system.

% % % \textit{D.	Capturing the data and error metrics}
% % \subsection{Capturing the data and error metrics}

% % Using the API provided by NDI, we can capture data from the system and command the robot suing the same script. The script configures the motion capture system and lets the user know that the system is ready to capture data. We perform a check to ensure that the tracking objects are tracked correctly. Once the user confirms that the objects can be tracked, the first set of joint variables are sent to the robot. After the robot has stopped moving, the user can position the pointer needle such that the robot tip and needle tip are coincident to record the data. The script records the position and the orientation (as quaternions) for the two objects. This process is repeated till the robot has moved to all the designated locations. The final data is exported as a .csv file.

% % The positions and quaternions are used form the transformation matrix for each frame that is being tracked. The measured tip position and expected tip position will be recorded, and its corresponding error will be reported in the subsequence section.
% % % \AR{Need to add text explaining the transforms and what we are calculating to determine error?}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{img/transformation_2columns.pdf}
%     \caption{Kinematic verification workspace with frames of interest obtained by Polaris Vega. (Robot tip frame): the tip of the concentric tubes or end effector frame obtained by marker probe. (Robot base frame): defined at the center of structural frame cut-out, which can be obtained through CAD parameters of the orange 3D printed component.}
%     \label{fig:fig-transform}
% \end{figure*}
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\textwidth]{img/transforms_CTR_NDI.png}
%     \caption{\AR{Can replace this with a better picture later}}
%     \label{fig:fig-transform}
% \end{figure*}
